Privacy-Preserving Data Deduplication for Enhancing Federated Learning of Language Models (Extended Version)

Deduplication is a vital preprocessing step that enhances machine learning model performance and saves training time and energy. However, enhancing federated learning through deduplication poses challenges, especially regarding scalability and potential privacy violations if deduplication involves sharing all clients' data. In this paper, we address the problem of deduplication in a federated setup by introducing a pioneering protocol, Efficient Privacy-Preserving Multi-Party Deduplication (EP-MPD). It efficiently removes duplicates from multiple clients' datasets without compromising data privacy. EP-MPD is constructed in a modular fashion, utilizing two novel variants of the Private Set Intersection protocol. Our extensive experiments demonstrate the significant benefits of deduplication in federated learning of large language models. For instance, we observe up to 19.62\% improvement in perplexity and up to 27.95\% reduction in running time while varying the duplication level between 10\% and 30\%. EP-MPD effectively balances privacy and performance in federated learning, making it a valuable solution for large-scale applications.

==> sections/generic-protocol.tex <==

\begin{enumerate}


\item Each pair of distinct parties $P_i, P_{i+1}$ computes the intersection of their sets, yielding $S^{(i, i+1)}_{\cap}=S_{i}\cap S_{i+1}$, where $1\leq i\leq n$.  In this case, both parties learn $S^{(i, i+1)}_{\cap}$. 


\item each party $P_{j}$ (where $j$ is an even integer and $j\leq n$) updates its set by calling $\update(S_{\st j}, S^{(j, j+1)}_{\cap})\rightarrow S_{\st j}$. It sends $S_{\st j}$ to $TP_{\st j}$.



\item  $P_{j+1}$ sends $S_{\st j+1}$ to $TP_{\st j}$


\item $TP_{\st j}$ which computes $\hat{S}_j=S_{\st j} + S_{\st j+1}$. 



% \item each party $P_{j}$ (where $j$ is an even integer and $j\leq n$) sends set $S_{j}\setminus S^{(j, j+1)}_{\cap}$ to $TP_{j}$, while $P_{j+1}$ sends $S_{j+1}$ to $TP_{j}$, which computes $\hat{S}_j=S_{j}\setminus S^{(j, j+1)}_{\cap} + S_{j+1}$. 

% \item only $P_{j}$ updates its local set $S_{j}$ as follows: $S_{j}= S_{j}\setminus S^{(j, j+1)}_{\cap}$.  

\item $TP_{j}$ and $TP_{j+1}$ compute the intersection of their sets:
 $S_{\cap}= \hat{S}_j\cap \hat{S}_{j+1}= (S_{j}\setminus S^{(j, j+1)}_{\cap} + S_{j+1}) \cap (S_{j+2}\setminus S^{(j+2, j+3)}_{\cap} + S_{j+3})$. 


\item for each element $e$ in $S_{\cap}$:


\begin{enumerate}
    \item each party who has $e$ declares its index of the leaf node.
    \item each party $P_{j}$ which declared its index, excluding the party which has the greatest index, updates its local set $S_{j}$ by calling $\update(S_{\st j}, S_{\st \cap})\rightarrow S_{\st j}$.

\end{enumerate}
  

\item At this stage the union of the parties will not include any replica. 


\end{enumerate}

==> sections/informal-security-analysis.tex <==




\section{Informal Security Analysis}




\revision{
%
In our schemes, if TEE is corrupted by a semi-honest adversary, then the adversary will only learn the size of the intersection that each pair of clients from a different group has (as defined in Definition \ref{def::leakage}), and nothing more, as proven in Appendices \ref{sec::proof-of-EG-PSI-1} and \ref{sec::proof-of-EG-PSI-2}. 
%
 In our schemes, TEE never learns any secret information about the parties (such as their secret keys).  Our schemes allow different $n-1$ clients to collude with each other (where $n$ is the total number of clients). By such collusion, they will not learn anything beyond what the collection of the intersection of each pair of honest and corrupt clients’ sets will reveal. }


==> sections/intro_copy.tex <==
\VD{Vishnu TODO: Add more NLP references, rewrite accuracy part, add privacy aspect, copyright issues}


The application of machine learning (ML) has experienced rapid growth, becoming widely embraced by businesses due to its various benefits. 
%
As ML relies heavily on data, there is an inherent risk of privacy breaches associated with this process. 
%
% Machine learning is a data dependent process, and needless to say that there is always a risk of privacy leakage associated with this. 
Federated Learning (\fl) is one of the basic steps towards privacy-preserving ML that allows training across multiple decentralized devices without exchanging their data. 
%
In \fl, devices compute local models based on their individual data and then share the local model updates with a central  server. 
%
This server aggregates the updates to derive a global model that encapsulates the features of all the local data held by the individual devices \cite{fedml_intro}.


% that aggregates them to derive the global model that captures the feature of all the local data held by the individual devices \cite{fedml_intro}. 
%However, there are certain attack methods such as Inference attack \cite{membership-inference-attack-sp2017} and model inversion attack \cite{model_inversion_attack} that tries to compromise the data used in training the models. Therefore, it is necessary to add additional layers of security to protect the local data privacy.


The accuracy of a ML model is significantly influenced by the quality of the training data. The accuracy is not solely dependent on the volume of data but also on its cleanliness. Data generated from real-world applications often lacks organization, leading to issues such as missing values, typos, format mismatches, outliers, or duplicated entries within the raw dataset. To ensure meaningful learning, it is imperative that the collected data undergoes a thorough data cleaning process \cite{ICbook19}.



% Accuracy of a machine learning model is very much dependent on the training data -- it not only depends on high volume of datasets, but also the quality of the training data highly influences the accuracy. 
% For instance, training with too many outliers will significantly affect the accuracy and could result in inaccurate inferences. Therefore, it is important to preprocess the data before the training so that the training data is free from outliers as much as possible.
%
% The data generated from various real-world applications is often unorganized and the (raw) dataset may contain errors (missing values, typos, format mismatch, etc.), outliers or duplicated entries. For a meaningful learning, the collected data must go through data cleaning process \cite{ICbook19}.

The presence of numerous duplicates in datasets significantly impacts accuracy. Duplicates prohibit the model's learning to be general -- model tends to memorize the output. Hence, preprocessing the data before training is crucial, with a key step being the removal of duplicates. This process, known as deduplication, is essential for enhancing the quality of the dataset and improving the accuracy of ML models. 


% Having too many duplicates in the datasets affects the accuracy greatly. Therefore, it is vital to preprocess the data before the training and remove duplicates as much as possible -- the process of removing duplicates is known as deduplication. 

% As demonstrated by Lee et al. \cite{lee-etal-2022-deduplicating}, duplicates can have negative affect on the overall learning procedure in a machine learning setup and pressed for the need of deduplucation before the training. 


As demonstrated by Lee et al. \cite{lee-etal-2022-deduplicating}, duplicates can adversely affect the overall learning process. Their findings underscore the importance of deduplication before training to mitigate such negative impacts and ensure the efficacy of the learning procedure.




In their case study focusing on language modeling datasets, Lee et al. investigated the C4 (Colossal Clean Crawled Corpus) dataset introduced by Raffel et al \cite{Raffel-C4}. 
%
They discovered a 61-word sequence within C4  that was repeated 61,036 times verbatim in the training dataset and 61 times in the validation set. They observed that train-test set overlap led to overestimating the model accuracy and a biased model selection. 

Deduplicating datasets not only improves the accuracy of learning but also enhances efficiency in various aspects.  By removing duplicates, it reduces CPU time and minimizes training costs in terms of time, money, and environmental resources. This streamlined process optimizes resource utilization and contributes to more sustainable ML  practices \cite{BGMS21,SGM19,Patterson-etal-carbon19}. Sustainable development is a global priority, and aligning ML practices with this theme is crucial.


% Considering the world's current emphasis on sustainable development, energy-efficient machine learning aligns well with this imperative.



 % Deduplication of datasets makes learning much more efficient too -- it saves CPU time and reduces the training cost in terms of time, money, and environment \cite{BGMS21,SGM19,Patterson-etal-carbon19}. 
 
 
 % \SuS{these references are from \cite{lee-etal-2022-deduplicating}, need to recheck before finalizing the paper.} 
 
 
 % Considering the world's current emphasis on sustainable development, energy-efficient machine learning aligns well with this imperative. 
 %
 % Given that the world is now more focused in sustainable developments,  energy-efficient machine learning is quite in line with this theme. 



 
 It was also observed in \cite{lee-etal-2022-deduplicating} that deduplication did not degrade perplexity, a metric used to evaluate how accurately a model predicts test samples (where lower scores are better). Interestingly, in certain instances, it even decreased perplexity by up to $10\%$. 
 
 
 % rather in some cases, it reduced perplexity by $10\%$.

Based on the discussions thus far, it is evident that deduplication offers numerous benefits, highlighting the importance of conducting deduplication prior to training. 
%
%As per the discussions so far, it is now evident that deduplication brings benefit in many ways, and so it is important to do deduplication before the training. 
%
% Since machine learning requires processing of data, therefore, it is crucial to take care of any privacy issues that could arise during the training or post the model preparation. 
%
There are several real-world applications which involve training with multiple entities/devices in the \fl setup such as healthcare \cite{ACKAE22}, smart city \cite{sensor}, and edge computing \cite{XYTWL2021}. Some of these applications are such that there is a good possibility of duplicates in the local training data across multiple devices. 

For example, Google keyboard  suggestions based on user's text query \cite{google_keyboard,BIKMMPRS17} applies \fl to train  local models in Android phones that later are aggregated to a global model. It is clear that there will be many text queries typed by the keyboards across multiple phones are the same. Therefore, text data in different mobile phones generated by these queries will have huge number of duplicates. 

Likewise, when we consider the application of \fl in smart city contexts, where sensor devices gather data throughout the city, it is likely that multiple sensors will capture identical data. 
%
% Similarly, if we consider \fl application in smart city applications where sensor devices collect data across the smart city, and here too there is a good chance that many sensors will collect the same data. 
%
For instance, sensors that are close to each other collecting environmental data may not have much variation in their collected data. 

In general, devices connected to an IoT network may collect similar data and contain many duplicates \cite{WHZW22}, which is true for both Industrial IoT (IIoT) and home IoT. 
%
% Furthermore, many IoT devices are resource constrained, if deduplication can significantly reduce the size of the training data for these devices, then these devices will be able to train the data faster and efficiently with their limited resources which could have been a heavier task had those duplicates remain in their dataset.
%
Moreover, considering that many IoT devices have limited resources, deduplication could substantially diminish the size of training data. Consequently, these devices would be capable of training data more swiftly and efficiently within their constraints. Without deduplication, managing duplicate data would impose a heavier burden on these devices.

Hence, for an efficient \fl process in the mentioned applications where duplicates are prevalent among the respective datasets, participating devices must first undergo deduplication.



% Therefore, an efficient federated learning involving the above mentioned  applications where duplicates occur among the respective datasets needs participating devices run deduplication first and then train.


When a data owner solely intends to remove duplicates from their own dataset, the privacy risk is minimal since the data is entirely under the owner's control. 
%
% If a data owner wants to remove duplicates from their own dataset only, the risk in terms of privacy is minimal as the data is completely possessed by the owner. 
%
In the context of FL, the scenario shifts significantly when deduplication is introduced. Multiple devices participating in FL may possess overlapping data, even after deduplicating their individual datasets. If they aim to deduplicate the combined dataset, one approach could involve sharing their raw data with each other and checking for intersections. However, this approach compromises the privacy guarantee of \fl. 


% This scenario completely changes when deduplication is considered in \fl setup. Two devices which are participtaing in a federated learning process, may share common data (even after deduplicating their own dataset). If they want to deduplicate the union of their data, then one possible way is to share each other's data and check the intersection. However, this immediately breaks the privacy guarantee of \fl. 



Hence, there is a necessity for privacy-preserving deduplication in the \fl setup, wherein participating devices would collaboratively deduplicate the combined datasets while maintaining the privacy of each individual dataset.

% Therefore, there is a need for privacy preserving deduplication in the \fl setup where participating devices would collaboratively deduplicate the union of their datasets keeping every individual dataset private.


This paper demonstrates how deduplication can be executed in a \fl setting without compromising the privacy of the data belonging to the individual devices engaged in the learning process. 


\subsection{Overview of Privacy-Preserving Deduplication in \fl}


Consider nodes $D_{\st 1}, \ldots, D_{\st n}$ are involved in a \fl, where each $D_{\st i}$ has a dataset $S_{\st i}$.  
%
Effectively, the training in \fl is conducted on the union of these datasets, i.e., $\bigcup\limits_{\st i=1}^{\st n} S_{\st i}$. 
%
If intersections exist among the datasets, \fl will  incorporate duplicates, leading to the drawbacks discussed earlier. %Hence, eliminating duplicates from training datasets is crucial without compromising users' data privacy.



% However, if there are  intersections between sets, this means the \fl training has been done on duplicates and the final model will suffer from the drawbacks due to duplicates in training datasets as discussed in the introduction. So, it is important to get rid of the duplicates from the training datasets without harming the users' data privacy. 

Let us initially consider  two nodes: $D_{\st 1}$ and $D_{\st 2}$, each with  datasets $S_{\st 1}$ and $S_{\st 2}$, respectively. If the intersection $S_{\st 1} \cap S_{\st 2}$ is nonempty, then training individually on $S_{\st 1}$ and $S_{\st 2}$ will mean training twice on $S_{\st 1} \cap S_{\st 2}$. The duplicate $S_{\st 1} \cap S_{\st 2}$ should be avoided, and that should be done without harming the data privacy of both $D_{\st 1}$ and $D_{\st 2}$. Our solution applies private set intersection (PSI) which securely finds intersection of $S_{\st 1}$ and $S_{\st 2}$ without revealing any other elements. 
%
Once $D_{\st 1}$ and $D_{\st 2}$ learn $S_{\st 1}\cap S_{\st 2}$ through PSI, $D_{\st 1}$ will train on $S_{\st 1}' = S_{\st 1} \setminus S_{\st 1} \cap S_{\st 2}$ and $D_{\st 2}$ will train on $S_{\st 2}$. 

According to set theory, it holds that $S_{\st 1}'\cup S_{\st 2} = S_{\st 1} \cup S_{\st 2}$. Hence, resulting \fl model remains as intended, while the training process is devoid of duplicates, thus avoiding associated drawbacks.

The scenario with two nodes seems straightforward. However, when more than two nodes participate, it becomes somewhat complicated. 

We now consider $n$ nodes $D_{\st 1}, \ldots, D_{\st n}$, where each node $D_{\st i}$ has a set $S_{\st i}$,  $\forall i, 1\leq i\leq n$, and  $n > 2$. 
 

% having sets $S_{\st 1}, \ldots, S_{\st n}$, respectively, where $n > 2$.


Following the two-node case, one might be tempted to (i) apply multi-party PSI to $n$ nodes, (ii)  find their intersection $I_{\st n}$, and (iii) let node $D_{\st 1}$ train on $S_{\st 1}' = S_{\st 1} \setminus I_{\st n}$, and rest of the nodes train on their own dataset $S_{\st i}$. This method will remove the duplicates that exist across all the nodes. However, this will not detect and remove the duplicates that exist among a subset of nodes. For instance, if there is $k$-sbuset ($k < n$) with a large intersection $I_{\st k}$, then $I_{\st k}$ will remain in the full training dataset $S_{\st 1}'\bigcup (\bigcup\limits_{\st i = 2}^{\st n} S_{\st i})$ as duplicates. 
%
Therefore, a generic multi-party PSI does not help in this case. So we need to consider nodes pairwise and remove the duplicates accordingly. %To be precise, we first need to run PSI among all possible pair of nodes.
%
%- $n \choose 2$ in total. 


\subsection{Our Contributions}


In this paper, we introduce an efficient privacy-preserving multi-party deduplication mechanism, called Duplication Eliminator (\epmpd). 
%
It enables datasets $S_{\st 1}, \ldots, S_{\st n}$ from various nodes (potentially containing duplicates) to be updated into new datasets $S_{\st 1}', \ldots, S_{\st n}'$. \epmpd ensures that  the union of the datasets before and after update are equal and the updated datasets are devoid of duplicates, i.e., $\bigcup\limits_{\st i = 1}^{\st n} S_{\st i}' = \bigcup\limits_{\st i = 1}^{\st n} S_i$, where $S_{\st i}' \cap S_{\st j}' = \emptyset, i \ne j$. 

We construct \epmpd in a modular fashion. 
%
Initially, we introduce two new PSIs, each capable of \textit{efficiently} identifying pairwise intersections among $n$ nodes. 
%
One of these PSIs leverages highly efficient symmetric-key primitives but requires continuous involvement of trusted hardware throughout the protocol. In contrast, the other PSI relies on asymmetric-key primitives, which are less efficient but require minimal engagement with secure hardware.

%
Subsequently, we demonstrate how \epmpd can be constructed using either of the aforementioned PSIs. We formally define and prove the security of \epmpd within the simulation-based paradigm. 





==> sections/tree-clusters.tex <==

\section{Clients Formation in \epmpd}\label{secc:clients-formation}

Figure \ref{fig::clients-formation} shows how clients are grouped at different levels of the tree, when there are $8$ clients. 

\begin{figure}[ht]
    \centering
    %\renewcommand{\arraystretch}{.02}
    \begin{subfigure}{0.47\textwidth}
        \centering
        \includegraphics[width=\linewidth, height=4cm]{Diag-1.pdf}
        \caption{Demonstration of clients joining various groups and clusters at level 1.}\label{fig:Diag-1}
    \end{subfigure}
%
    %\vspace{10pt} % Adjust the vertical space between top and bottom figures
%
    \begin{subfigure}{0.47\textwidth}
    %\begin{subfigure}{4cm}
        \centering
        %\includegraphics[width=\linewidth]{Diag-2.pdf}
        \includegraphics[width=\linewidth, height=4cm]{Diag-2.pdf}
        \caption{Illustration of clients joining various groups and clusters at  level 2.}\label{fig:Diag-2}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.47\textwidth}
        \centering
        \includegraphics[width=\linewidth, height=4cm]{Diag-3.pdf}
        \caption{Depiction of how clients become part of diverse groups and clusters at  level 3.}\label{fig:Diag-3}
    \end{subfigure}

    \caption{The process of eight clients forming clusters and groups at various levels of a binary tree. At each level, clients belonging to groups $\gr_{\st 0}$ and $\gr_{\st 1}$ within the same cluster initiate \egpsi, followed by the updating of their respective local sets.}\label{fig::clients-formation}
\end{figure}

==> sections/type3.tex <==
\section{Symmetric Key Based \egpsi without Third Party (Type III)}

In Figure \ref{fig:EG-PSI-random-elem}, we introduce an optimized version of group PSI tailored for scenarios where set elements are uniformly distributed across the universe of elements. This is particularly applicable in cases such as sets containing credentials or PINs.

\begin{figure}[!h]
\setlength{\fboxsep}{.9pt}
\begin{center}
    \begin{tcolorbox}[enhanced, left=0mm,
    drop fuzzy shadow southwest,
    colframe=black,colback=white]
    % {\small{

%\vspace{-2.2mm}
\begin{itemize}[leftmargin=4.2mm]

\item \textit{Parties}. Clients in group $\gr_{\st 0}:\{\cl_{\st 0,1},...,\cl_{\st 0,m}\}$, and clients in group $\gr_{\st 1}:\{\cl_{\st 1,1},...,\cl_{\st 1,m}\}$. 

\item \textit{Inputs}. Sets $\set_{\st 0,1}, ..., \set_{\st 0, m}, \set_{\st 1,1},..., \set_{\st 1,m}$, where each $\set_{\st j,i}$ belongs to client $\cl_{\st j,i}$, $0\leq j \leq 1$ and $1\leq i \leq m$.

 \item\textit{Outputs}. $\vec{v}_{\st 0, i}$ to $\cl_{\st 0, i}$, where $\vec{v}_{\st 0, i}=\Big[[\set_{\st 0, i}\cap \set_{\st 1, 1}],...,[\set_{\st 0, i}\cap \set_{\st 1, m}]\Big]$. 
 
\noindent\rule{\textwidth}{0.1pt}


\end{itemize}
%
\begin{enumerate}[leftmargin=5.2mm]
\item \underline{\textit{Setup}.}
\begin{enumerate}[leftmargin=5.2mm]
%

\item each $\cl_{\st 1, i}$ takes the following steps:

\begin{enumerate}

\item for every element $e \in S_{1, i}$ decides a key $k_e = Hash(e)$ and encrypts that $e$ as $\PRP(k_{e}, e)$. Let $\set'_{\st 1, i}$ contain the encrypted set elements of $\cl_{\st 1, i}$.

\end{enumerate}

\item $\cl_{\st 1, i}$ sends their respective sets $\set'_{\st 1, i}$ to all the clients $\cl_{\st 0, i}$.

\end{enumerate}

\item \underline{\textit{Finding the  Intersection}.} Each $\cl_{\st 0, i}$ takes the following steps. 

\begin{enumerate} 
%
\item constructs a vector $\vec{v}_{\st 0,i}=[\vec{v}_{\st 0,i, 1},..., \vec{v}_{\st 0,i, m}]$, where each vector in $\vec{v}_{\st 0,i}$ is initially empty. 

\item for every element $e \in S_{0, i}$ determines $k_e = Hash(e)$ and $\PRP(k_{e}, e)$,  
\begin{itemize}
\item if  $\PRP(k_{e}, e) \in \set'_{\st 1, \ell}$, appends $e$ to $\vec{v}_{\st 0,i, \ell}$ 

 

\end{itemize}

\item considers $\vec{v}_{\st 0,i}$ as the result.


\end{enumerate}

\end{enumerate}
% }   }
\end{tcolorbox}
\end{center}
%\vspace{-3mm}
\caption{Variant of Efficient Group PSI (Type III).}
% \vspace{-3mm}
\label{fig:EG-PSI-random-elem}
\end{figure}
%\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


